Overcoming Common Flaws in the Evaluation of Selective Classification Systems

Selective Classification, wherein models can reject low-confidence predictions, promises reliable translation of machine-learning based classification systems to real-world scenarios such as clinical diagnostics. While current evaluation of these systems typically assumes fixed working points based on pre-defined rejection thresholds, methodological progress requires benchmarking the general performance of systems akin to the $\mathrm{AUROC}$ in standard classification. In this work, we define 5 requirements for multi-threshold metrics in selective classification regarding task alignment, interpretability, and flexibility, and show how current approaches fail to meet them. We propose the Area under the Generalized Risk Coverage curve ($\mathrm{AUGRC}$), which meets all requirements and can be directly interpreted as the average risk of undetected failures. We empirically demonstrate the relevance of $\mathrm{AUGRC}$ on a comprehensive benchmark spanning 6 data sets and 13 confidence scoring functions. We find that the proposed metric substantially changes metric rankings on 5 out of the 6 data sets.

==> tables/paper_results_augrc_original.tex <==
\begin{tabular}{ll?rr?xx?xx?rrrrrr?rrrrr?rrrr}
 & \multicolumn{1}{c}{} & \multicolumn{2}{c}{iWildCam} & \multicolumn{2}{c}{BREEDS} & \multicolumn{2}{c}{CAMELYON} & \multicolumn{6}{c}{CIFAR-100} & \multicolumn{5}{c}{CIFAR-10} & \multicolumn{4}{c}{SVHN} \\
 & study & iid & sub & iid & sub & iid & sub & iid & sub & cor & s-ncs & \multicolumn{2}{c?}{ns-ncs} & iid & cor & s-ncs & \multicolumn{2}{c?}{ns-ncs} & iid & \multicolumn{3}{c}{ns-ncs} \\
 & ncs-data set &  &  &  &  &  &  &  &  &  & c10 & svhn & ti &  &  & c100 & svhn & ti &  & c10 & c100 & ti \\
\midrule
MSR & CNN & {\cellcolor[HTML]{FEE5CC}} \color[HTML]{000000} 48.0 & {\cellcolor[HTML]{FFF3E7}} \color[HTML]{000000} 55.0 & {\cellcolor[HTML]{FEDDBC}} \color[HTML]{000000} 6.86 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1} 117 & {\cellcolor[HTML]{FDD5AB}} \color[HTML]{000000} 8.13 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000} 91.3 & {\cellcolor[HTML]{FEE6CF}} \color[HTML]{000000} 54.6 & {\cellcolor[HTML]{FFEEDD}} \color[HTML]{000000} 150 & {\cellcolor[HTML]{FDC48F}} \color[HTML]{000000} 187 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 210 & {\cellcolor[HTML]{FDAC67}} \color[HTML]{000000} 334 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1} 203 & {\cellcolor[HTML]{F67824}} \color[HTML]{F1F1F1} 4.93 & {\cellcolor[HTML]{DE5005}} \color[HTML]{F1F1F1} 67.9 & {\cellcolor[HTML]{F3701B}} \color[HTML]{F1F1F1} 166 & {\cellcolor[HTML]{FDCB9B}} \color[HTML]{000000} 291 & {\cellcolor[HTML]{FDB170}} \color[HTML]{000000} 154 & {\cellcolor[HTML]{FFF2E5}} \color[HTML]{000000} 3.44 & {\cellcolor[HTML]{BE3F02}} \color[HTML]{F1F1F1} 48.5 & {\cellcolor[HTML]{A63603}} \color[HTML]{F1F1F1} 48.2 & {\cellcolor[HTML]{F36E19}} \color[HTML]{F1F1F1} 48.6 \\
MLS & CNN & {\cellcolor[HTML]{FD9B50}} \color[HTML]{000000} 60.3 & {\cellcolor[HTML]{FDD5AD}} \color[HTML]{000000} 62.4 & {\cellcolor[HTML]{8A2B04}} \color[HTML]{F1F1F1} 9.28 & {\cellcolor[HTML]{9E3303}} \color[HTML]{F1F1F1} 121 & {\cellcolor[HTML]{FDD5AB}} \color[HTML]{000000} 8.13 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000} 91.3 & {\cellcolor[HTML]{D14501}} \color[HTML]{F1F1F1} 65.6 & {\cellcolor[HTML]{FEE7D0}} \color[HTML]{000000} 155 & {\cellcolor[HTML]{EB610F}} \color[HTML]{F1F1F1} 200 & {\cellcolor[HTML]{FDD1A3}} \color[HTML]{000000} 213 & {\cellcolor[HTML]{F26C16}} \color[HTML]{F1F1F1} 337 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 195 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 5.56 & {\cellcolor[HTML]{D14501}} \color[HTML]{F1F1F1} 68.4 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 163 & {\cellcolor[HTML]{FEEDDC}} \color[HTML]{000000} 288 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 150 & {\cellcolor[HTML]{FDCA99}} \color[HTML]{000000} 3.97 & {\cellcolor[HTML]{FEEDDB}} \color[HTML]{000000} 46.5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 46.1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 46.6 \\
PE & CNN & {\cellcolor[HTML]{FEE4CA}} \color[HTML]{000000} 48.2 & {\cellcolor[HTML]{FFF2E6}} \color[HTML]{000000} 55.2 & {\cellcolor[HTML]{FEDCBB}} \color[HTML]{000000} 6.87 & {\cellcolor[HTML]{FDA762}} \color[HTML]{000000} 116 & {\cellcolor[HTML]{FDD5AB}} \color[HTML]{000000} 8.13 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000} 91.3 & {\cellcolor[HTML]{FDD4AA}} \color[HTML]{000000} 56.4 & {\cellcolor[HTML]{FFEEDD}} \color[HTML]{000000} 150 & {\cellcolor[HTML]{FDB87C}} \color[HTML]{000000} 188 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 210 & {\cellcolor[HTML]{FDC189}} \color[HTML]{000000} 333 & {\cellcolor[HTML]{FD9E54}} \color[HTML]{000000} 202 & {\cellcolor[HTML]{F87D29}} \color[HTML]{F1F1F1} 4.91 & {\cellcolor[HTML]{EB610F}} \color[HTML]{F1F1F1} 67.2 & {\cellcolor[HTML]{FDA762}} \color[HTML]{000000} 165 & {\cellcolor[HTML]{FDD9B4}} \color[HTML]{000000} 290 & {\cellcolor[HTML]{FEDCBB}} \color[HTML]{000000} 152 & {\cellcolor[HTML]{FFF2E5}} \color[HTML]{000000} 3.44 & {\cellcolor[HTML]{F4721E}} \color[HTML]{F1F1F1} 47.9 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1} 47.5 & {\cellcolor[HTML]{FDA159}} \color[HTML]{000000} 48.0 \\
MCD-MSR & CNN & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 42.8 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 54.3 & {\cellcolor[HTML]{FDDBB8}} \color[HTML]{000000} 6.89 & {\cellcolor[HTML]{FDA762}} \color[HTML]{000000} 116 & {\cellcolor[HTML]{FEE9D3}} \color[HTML]{000000} 5.64 & {\cellcolor[HTML]{FEE3C8}} \color[HTML]{000000} 95.1 & {\cellcolor[HTML]{FFF1E4}} \color[HTML]{000000} 53.1 & {\cellcolor[HTML]{FFF4E8}} \color[HTML]{000000} 146 & {\cellcolor[HTML]{FFF2E6}} \color[HTML]{000000} 176 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 210 & {\cellcolor[HTML]{F98230}} \color[HTML]{F1F1F1} 336 & {\cellcolor[HTML]{FD9E54}} \color[HTML]{000000} 202 & {\cellcolor[HTML]{FDBE84}} \color[HTML]{000000} 4.56 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 60.4 & {\cellcolor[HTML]{F3701B}} \color[HTML]{F1F1F1} 166 & {\cellcolor[HTML]{FD9649}} \color[HTML]{000000} 294 & {\cellcolor[HTML]{F9802D}} \color[HTML]{F1F1F1} 156 & {\cellcolor[HTML]{FFF4E9}} \color[HTML]{000000} 3.40 & {\cellcolor[HTML]{FDB06E}} \color[HTML]{000000} 47.3 & {\cellcolor[HTML]{F9812E}} \color[HTML]{F1F1F1} 47.4 & {\cellcolor[HTML]{FDA965}} \color[HTML]{000000} 47.9 \\
MCD-PE & CNN & {\cellcolor[HTML]{FFF4E8}} \color[HTML]{000000} 43.4 & {\cellcolor[HTML]{FFF3E6}} \color[HTML]{000000} 55.1 & {\cellcolor[HTML]{FDD6AE}} \color[HTML]{000000} 6.98 & {\cellcolor[HTML]{FDA762}} \color[HTML]{000000} 116 & {\cellcolor[HTML]{FEE9D3}} \color[HTML]{000000} 5.64 & {\cellcolor[HTML]{FEE3C8}} \color[HTML]{000000} 95.1 & {\cellcolor[HTML]{FDD2A6}} \color[HTML]{000000} 56.6 & {\cellcolor[HTML]{FFF4E8}} \color[HTML]{000000} 146 & {\cellcolor[HTML]{FEEBD7}} \color[HTML]{000000} 179 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 210 & {\cellcolor[HTML]{FD974A}} \color[HTML]{000000} 335 & {\cellcolor[HTML]{FEDCB9}} \color[HTML]{000000} 198 & {\cellcolor[HTML]{FD9E54}} \color[HTML]{000000} 4.73 & {\cellcolor[HTML]{FFF3E7}} \color[HTML]{000000} 60.6 & {\cellcolor[HTML]{FDD9B4}} \color[HTML]{000000} 164 & {\cellcolor[HTML]{FDA762}} \color[HTML]{000000} 293 & {\cellcolor[HTML]{FDCA99}} \color[HTML]{000000} 153 & {\cellcolor[HTML]{FFF0E2}} \color[HTML]{000000} 3.47 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 46.3 & {\cellcolor[HTML]{FEE6CF}} \color[HTML]{000000} 46.4 & {\cellcolor[HTML]{FEEAD6}} \color[HTML]{000000} 46.9 \\
MCD-MI & CNN & {\cellcolor[HTML]{FFF3E6}} \color[HTML]{000000} 43.7 & {\cellcolor[HTML]{FEE9D3}} \color[HTML]{000000} 58.1 & {\cellcolor[HTML]{FDBF86}} \color[HTML]{000000} 7.28 & {\cellcolor[HTML]{F3701B}} \color[HTML]{F1F1F1} 118 & {\cellcolor[HTML]{FEE6CE}} \color[HTML]{000000} 6.13 & {\cellcolor[HTML]{FDD3A7}} \color[HTML]{000000} 101 & {\cellcolor[HTML]{FDA660}} \color[HTML]{000000} 59.4 & {\cellcolor[HTML]{FFF1E3}} \color[HTML]{000000} 148 & {\cellcolor[HTML]{FEDCBB}} \color[HTML]{000000} 182 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000} 211 & {\cellcolor[HTML]{FDC189}} \color[HTML]{000000} 333 & {\cellcolor[HTML]{FEE6CF}} \color[HTML]{000000} 197 & {\cellcolor[HTML]{F26D17}} \color[HTML]{F1F1F1} 4.99 & {\cellcolor[HTML]{FD9F56}} \color[HTML]{000000} 64.9 & {\cellcolor[HTML]{C54102}} \color[HTML]{F1F1F1} 167 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 302 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 161 & {\cellcolor[HTML]{FEECDA}} \color[HTML]{000000} 3.55 & {\cellcolor[HTML]{FDCE9E}} \color[HTML]{000000} 47.0 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1} 47.7 & {\cellcolor[HTML]{FD9141}} \color[HTML]{000000} 48.2 \\
ConfidNet & CNN & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 82.0 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 91.2 & {\cellcolor[HTML]{FDDBB8}} \color[HTML]{000000} 6.89 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1} 117 & {\cellcolor[HTML]{FFF0E1}} \color[HTML]{000000} 4.36 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 86.1 & {\cellcolor[HTML]{FDC590}} \color[HTML]{000000} 57.5 & {\cellcolor[HTML]{FEE8D2}} \color[HTML]{000000} 154 & {\cellcolor[HTML]{FD9F56}} \color[HTML]{000000} 192 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000} 214 & {\cellcolor[HTML]{B13A03}} \color[HTML]{F1F1F1} 340 & {\cellcolor[HTML]{FDC088}} \color[HTML]{000000} 200 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000} 4.70 & {\cellcolor[HTML]{FD9243}} \color[HTML]{000000} 65.4 & {\cellcolor[HTML]{FDA762}} \color[HTML]{000000} 165 & {\cellcolor[HTML]{FDCB9B}} \color[HTML]{000000} 291 & {\cellcolor[HTML]{FDCA99}} \color[HTML]{000000} 153 & {\cellcolor[HTML]{FFF3E6}} \color[HTML]{000000} 3.43 & {\cellcolor[HTML]{AE3903}} \color[HTML]{F1F1F1} 48.6 & {\cellcolor[HTML]{8B2C04}} \color[HTML]{F1F1F1} 48.4 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1} 48.8 \\
DG-MCD-MSR & CNN & {\cellcolor[HTML]{FFF2E5}} \color[HTML]{000000} 43.9 & {\cellcolor[HTML]{FEE3C8}} \color[HTML]{000000} 59.6 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 6.31 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 112 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 3.47 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 149 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 52.5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 145 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 175 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 210 & {\cellcolor[HTML]{F98230}} \color[HTML]{F1F1F1} 336 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1} 203 & {\cellcolor[HTML]{FD9B50}} \color[HTML]{000000} 4.75 & {\cellcolor[HTML]{FFF1E3}} \color[HTML]{000000} 60.8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 168 & {\cellcolor[HTML]{F3701B}} \color[HTML]{F1F1F1} 296 & {\cellcolor[HTML]{BD3E02}} \color[HTML]{F1F1F1} 159 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 3.38 & {\cellcolor[HTML]{FD9243}} \color[HTML]{000000} 47.6 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1} 47.7 & {\cellcolor[HTML]{FDA159}} \color[HTML]{000000} 48.0 \\
DG-Res & CNN & {\cellcolor[HTML]{F36F1A}} \color[HTML]{F1F1F1} 66.5 & {\cellcolor[HTML]{FDCFA0}} \color[HTML]{000000} 63.8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 9.39 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 122 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 3.46 & {\cellcolor[HTML]{F36F1A}} \color[HTML]{F1F1F1} 124 & {\cellcolor[HTML]{E4580A}} \color[HTML]{F1F1F1} 64.3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 230 & {\cellcolor[HTML]{FD9141}} \color[HTML]{000000} 194 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000} 215 & {\cellcolor[HTML]{FEECDA}} \color[HTML]{000000} 330 & {\cellcolor[HTML]{FEE6CF}} \color[HTML]{000000} 197 & {\cellcolor[HTML]{FDD7B1}} \color[HTML]{000000} 4.40 & {\cellcolor[HTML]{FDBB81}} \color[HTML]{000000} 63.8 & {\cellcolor[HTML]{C54102}} \color[HTML]{F1F1F1} 167 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 287 & {\cellcolor[HTML]{FEEAD6}} \color[HTML]{000000} 151 & {\cellcolor[HTML]{FDBB81}} \color[HTML]{000000} 4.09 & {\cellcolor[HTML]{FEDCB9}} \color[HTML]{000000} 46.8 & {\cellcolor[HTML]{FFF0E2}} \color[HTML]{000000} 46.2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 46.6 \\
Devries et al. & CNN & {\cellcolor[HTML]{FD9243}} \color[HTML]{000000} 61.7 & {\cellcolor[HTML]{F87E2B}} \color[HTML]{F1F1F1} 74.7 & {\cellcolor[HTML]{F16813}} \color[HTML]{F1F1F1} 8.24 & {\cellcolor[HTML]{C54102}} \color[HTML]{F1F1F1} 120 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 24.3 & {\cellcolor[HTML]{932F03}} \color[HTML]{F1F1F1} 145 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 69.6 & {\cellcolor[HTML]{FFEEDD}} \color[HTML]{000000} 150 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 214 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 222 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 342 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 211 & {\cellcolor[HTML]{FDBB81}} \color[HTML]{000000} 4.57 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 70.8 & {\cellcolor[HTML]{F3701B}} \color[HTML]{F1F1F1} 166 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 287 & {\cellcolor[HTML]{FEDCBB}} \color[HTML]{000000} 152 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 5.56 & {\cellcolor[HTML]{DB4A02}} \color[HTML]{F1F1F1} 48.3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 48.5 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 49.9 \\
TEMP-MLS & CNN & {\cellcolor[HTML]{FEE4CA}} \color[HTML]{000000} 48.2 & {\cellcolor[HTML]{FFF3E6}} \color[HTML]{000000} 55.1 & {\cellcolor[HTML]{FEDDBC}} \color[HTML]{000000} 6.86 & {\cellcolor[HTML]{FDA762}} \color[HTML]{000000} 116 & {\cellcolor[HTML]{FDD5AB}} \color[HTML]{000000} 8.13 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000} 91.3 & {\cellcolor[HTML]{FEE5CB}} \color[HTML]{000000} 54.8 & {\cellcolor[HTML]{FFEEDD}} \color[HTML]{000000} 150 & {\cellcolor[HTML]{FDC48F}} \color[HTML]{000000} 187 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 210 & {\cellcolor[HTML]{FDC189}} \color[HTML]{000000} 333 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1} 203 & {\cellcolor[HTML]{F77A27}} \color[HTML]{F1F1F1} 4.92 & {\cellcolor[HTML]{E45709}} \color[HTML]{F1F1F1} 67.6 & {\cellcolor[HTML]{F3701B}} \color[HTML]{F1F1F1} 166 & {\cellcolor[HTML]{FDCB9B}} \color[HTML]{000000} 291 & {\cellcolor[HTML]{FDCA99}} \color[HTML]{000000} 153 & {\cellcolor[HTML]{FFF2E5}} \color[HTML]{000000} 3.44 & {\cellcolor[HTML]{DB4A02}} \color[HTML]{F1F1F1} 48.3 & {\cellcolor[HTML]{D94801}} \color[HTML]{F1F1F1} 47.9 & {\cellcolor[HTML]{F9802D}} \color[HTML]{F1F1F1} 48.4 \\
DG-PE & CNN & {\cellcolor[HTML]{FDD3A7}} \color[HTML]{000000} 52.0 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000} 69.7 & {\cellcolor[HTML]{FFF5EA}} \color[HTML]{000000} 6.33 & {\cellcolor[HTML]{FDD9B4}} \color[HTML]{000000} 114 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 3.46 & {\cellcolor[HTML]{F5741F}} \color[HTML]{F1F1F1} 123 & {\cellcolor[HTML]{FEE0C3}} \color[HTML]{000000} 55.2 & {\cellcolor[HTML]{FEEDDB}} \color[HTML]{000000} 151 & {\cellcolor[HTML]{FDC590}} \color[HTML]{000000} 186 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 210 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 329 & {\cellcolor[HTML]{FEE6CF}} \color[HTML]{000000} 197 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 4.09 & {\cellcolor[HTML]{FDD2A6}} \color[HTML]{000000} 62.9 & {\cellcolor[HTML]{C54102}} \color[HTML]{F1F1F1} 167 & {\cellcolor[HTML]{FEEDDC}} \color[HTML]{000000} 288 & {\cellcolor[HTML]{FDB170}} \color[HTML]{000000} 154 & {\cellcolor[HTML]{FFF4E8}} \color[HTML]{000000} 3.41 & {\cellcolor[HTML]{8A2B04}} \color[HTML]{F1F1F1} 48.9 & {\cellcolor[HTML]{8B2C04}} \color[HTML]{F1F1F1} 48.4 & {\cellcolor[HTML]{EF6612}} \color[HTML]{F1F1F1} 48.7 \\
DG-TEMP-MLS & CNN & {\cellcolor[HTML]{FDD2A6}} \color[HTML]{000000} 52.2 & {\cellcolor[HTML]{FDA159}} \color[HTML]{000000} 69.9 & {\cellcolor[HTML]{FFF4E8}} \color[HTML]{000000} 6.35 & {\cellcolor[HTML]{FDD9B4}} \color[HTML]{000000} 114 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 3.46 & {\cellcolor[HTML]{F5741F}} \color[HTML]{F1F1F1} 123 & {\cellcolor[HTML]{FEE2C7}} \color[HTML]{000000} 55.0 & {\cellcolor[HTML]{9C3203}} \color[HTML]{F1F1F1} 222 & {\cellcolor[HTML]{FDD3A9}} \color[HTML]{000000} 184 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000} 211 & {\cellcolor[HTML]{FEE1C4}} \color[HTML]{000000} 331 & {\cellcolor[HTML]{FDD1A3}} \color[HTML]{000000} 199 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000} 4.09 & {\cellcolor[HTML]{FDCE9E}} \color[HTML]{000000} 63.1 & {\cellcolor[HTML]{C54102}} \color[HTML]{F1F1F1} 167 & {\cellcolor[HTML]{FEEDDC}} \color[HTML]{000000} 288 & {\cellcolor[HTML]{FD994D}} \color[HTML]{000000} 155 & {\cellcolor[HTML]{FFF4E8}} \color[HTML]{000000} 3.41 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 49.0 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1} 48.5 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1} 48.8 \\
\bottomrule
\end{tabular}

==> tables/rank_comparison_joint_original.tex <==
\begin{tabular}{ll?*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}}
 & \multicolumn{1}{c}{} & \multicolumn{4}{c?}{iWildCam} & \multicolumn{4}{c?}{BREEDS} & \multicolumn{4}{c?}{CAMELYON} & \multicolumn{12}{c?}{CIFAR-100} & \multicolumn{10}{c?}{CIFAR-10} & \multicolumn{8}{c}{SVHN} \\
 & study & \multicolumn{2}{c?}{iid} & \multicolumn{2}{c?}{sub} & \multicolumn{2}{c?}{iid} & \multicolumn{2}{c?}{sub} & \multicolumn{2}{c?}{iid} & \multicolumn{2}{c?}{sub} & \multicolumn{2}{c?}{iid} & \multicolumn{2}{c?}{sub} & \multicolumn{2}{c?}{cor} & \multicolumn{2}{c?}{s-ncs} & \multicolumn{4}{c?}{ns-ncs} & \multicolumn{2}{c?}{iid} & \multicolumn{2}{c?}{cor} & \multicolumn{2}{c?}{s-ncs} & \multicolumn{4}{c?}{ns-ncs} & \multicolumn{2}{c?}{iid} & \multicolumn{6}{c}{ns-ncs} \\
 & ncs-data set & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{c10} & \multicolumn{2}{c?}{svhn} & \multicolumn{2}{c?}{ti} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{c100} & \multicolumn{2}{c?}{svhn} & \multicolumn{2}{c?}{ti} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{c10} & \multicolumn{2}{c?}{c100} & \multicolumn{2}{c}{ti} \\
 & metric & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ \\
\midrule
optimized both \\
\midrule
MSR & CNN & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{DD4D04}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 \\
MLS & CNN & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 \\
PE & CNN & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD994D}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 \\
MCD-MSR & CNN & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB170}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 \\
MCD-PE & CNN & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDCA99}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 \\
MCD-EE & CNN & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDCBB}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 \\
ConfidNet & CNN & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{BD3E02}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 \\
DG-MCD-MSR & CNN & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{F9802D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 \\
DG-Res & CNN & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEAD6}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 \\
Devries et al. & CNN & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 \\
TEMP-MLS & CNN & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{EF6612}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 \\
DG-PE & CNN & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{BD3E02}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 \\
DG-TEMP-MLS & CNN & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 \\
\midrule
optimized AUGRC \\
\midrule
MSR & CNN & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{DD4D04}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 \\
MLS & CNN & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 \\
PE & CNN & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD994D}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 \\
MCD-MSR & CNN & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB170}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 \\
MCD-PE & CNN & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDCA99}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 \\
MCD-EE & CNN & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDCBB}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 \\
ConfidNet & CNN & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{BD3E02}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 \\
DG-MCD-MSR & CNN & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{F9802D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 \\
DG-Res & CNN & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEAD6}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 \\
Devries et al. & CNN & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 \\
TEMP-MLS & CNN & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{EF6612}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 \\
DG-PE & CNN & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{BD3E02}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 \\
DG-TEMP-MLS & CNN & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 \\
\bottomrule
\end{tabular}

==> tables/rank_metric_comparison_aurc_to_augrc_optimized_augrc.tex <==
\begin{tabular}{ll?*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}}
 & \multicolumn{1}{c}{} & \multicolumn{4}{c?}{iWildCam} & \multicolumn{4}{c?}{BREEDS} & \multicolumn{4}{c?}{CAMELYON} & \multicolumn{12}{c?}{CIFAR-100} & \multicolumn{10}{c?}{CIFAR-10} & \multicolumn{8}{c}{SVHN} \\
 & study & \multicolumn{2}{c?}{iid} & \multicolumn{2}{c?}{sub} & \multicolumn{2}{c?}{iid} & \multicolumn{2}{c?}{sub} & \multicolumn{2}{c?}{iid} & \multicolumn{2}{c?}{sub} & \multicolumn{2}{c?}{iid} & \multicolumn{2}{c?}{sub} & \multicolumn{2}{c?}{cor} & \multicolumn{2}{c?}{s-ncs} & \multicolumn{4}{c?}{ns-ncs} & \multicolumn{2}{c?}{iid} & \multicolumn{2}{c?}{cor} & \multicolumn{2}{c?}{s-ncs} & \multicolumn{4}{c?}{ns-ncs} & \multicolumn{2}{c?}{iid} & \multicolumn{6}{c}{ns-ncs} \\
 & ncs-data set & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{c10} & \multicolumn{2}{c?}{svhn} & \multicolumn{2}{c?}{ti} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{c100} & \multicolumn{2}{c?}{svhn} & \multicolumn{2}{c?}{ti} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{c10} & \multicolumn{2}{c?}{c100} & \multicolumn{2}{c}{ti} \\
 & metric & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ \\
\midrule
MSR & CNN & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{DD4D04}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 \\
MLS & CNN & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 \\
PE & CNN & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD994D}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 \\
MCD-MSR & CNN & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB170}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 \\
MCD-PE & CNN & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDCA99}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 \\
MCD-EE & CNN & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDCBB}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 \\
ConfidNet & CNN & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{BD3E02}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 \\
DG-MCD-MSR & CNN & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{F9802D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 \\
DG-Res & CNN & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEAD6}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 \\
Devries et al. & CNN & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 \\
TEMP-MLS & CNN & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{EF6612}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 \\
DG-PE & CNN & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{BD3E02}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 \\
DG-TEMP-MLS & CNN & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 \\
\bottomrule
\end{tabular}

==> tables/rank_metric_comparison_aurc_to_augrc_optimized_both.tex <==
\begin{tabular}{ll?*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}h*{2}{r}}
 & \multicolumn{1}{c}{} & \multicolumn{4}{c?}{iWildCam} & \multicolumn{4}{c?}{BREEDS} & \multicolumn{4}{c?}{CAMELYON} & \multicolumn{12}{c?}{CIFAR-100} & \multicolumn{10}{c?}{CIFAR-10} & \multicolumn{8}{c}{SVHN} \\
 & study & \multicolumn{2}{c?}{iid} & \multicolumn{2}{c?}{sub} & \multicolumn{2}{c?}{iid} & \multicolumn{2}{c?}{sub} & \multicolumn{2}{c?}{iid} & \multicolumn{2}{c?}{sub} & \multicolumn{2}{c?}{iid} & \multicolumn{2}{c?}{sub} & \multicolumn{2}{c?}{cor} & \multicolumn{2}{c?}{s-ncs} & \multicolumn{4}{c?}{ns-ncs} & \multicolumn{2}{c?}{iid} & \multicolumn{2}{c?}{cor} & \multicolumn{2}{c?}{s-ncs} & \multicolumn{4}{c?}{ns-ncs} & \multicolumn{2}{c?}{iid} & \multicolumn{6}{c}{ns-ncs} \\
 & ncs-data set & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{c10} & \multicolumn{2}{c?}{svhn} & \multicolumn{2}{c?}{ti} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{c100} & \multicolumn{2}{c?}{svhn} & \multicolumn{2}{c?}{ti} & \multicolumn{2}{c?}{} & \multicolumn{2}{c?}{c10} & \multicolumn{2}{c?}{c100} & \multicolumn{2}{c}{ti} \\
 & metric & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ & $\alpha$ & $\beta$ \\
\midrule
MSR & CNN & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{DD4D04}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 \\
MLS & CNN & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 \\
PE & CNN & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD994D}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 \\
MCD-MSR & CNN & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB170}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 \\
MCD-PE & CNN & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDCA99}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 \\
MCD-EE & CNN & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDCBB}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 \\
ConfidNet & CNN & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{BD3E02}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 \\
DG-MCD-MSR & CNN & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{F9802D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 \\
DG-Res & CNN & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEAD6}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 \\
Devries et al. & CNN & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 \\
TEMP-MLS & CNN & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{EF6612}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 \\
DG-PE & CNN & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FD8E3D}} \color[HTML]{F1F1F1}   7 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{BD3E02}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 \\
DG-TEMP-MLS & CNN & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FEEBD8}} \color[HTML]{000000}   2 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{E95E0D}} \color[HTML]{F1F1F1}   9 & {\cellcolor[HTML]{FDD0A2}} \color[HTML]{000000}   4 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{F57520}} \color[HTML]{F1F1F1}   8 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FFF5EB}} \color[HTML]{000000}   1 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{FDA35C}} \color[HTML]{000000}   6 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{D84801}} \color[HTML]{F1F1F1}  10 & {\cellcolor[HTML]{FDB97D}} \color[HTML]{000000}   5 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{FEDFC0}} \color[HTML]{000000}   3 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  13 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{7F2704}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{993103}} \color[HTML]{F1F1F1}  12 & {\cellcolor[HTML]{B63C02}} \color[HTML]{F1F1F1}  11 \\
\bottomrule
\end{tabular}
